Arc-based Traffic Assignment: Equilibrium Characterization and Learning

Arc-based traffic assignment models (TAMs) are a popular framework for modeling traffic network congestion generated by self-interested travelers who sequentially select arcs based on their perceived latency on the network. However, existing arc-based TAMs either assign travelers to cyclic paths, or do not extend to networks with bi-directional arcs (or edges) between nodes. To overcome these difficulties, we propose a new modeling framework for stochastic arc-based TAMs. Given a traffic network with bidirectional arcs, we replicate its arcs and nodes to construct a directed acyclic graph (DAG), which we call the Condensed DAG (CoDAG) representation. Self-interested travelers sequentially select arcs on the CoDAG representation to reach their destination. We show that the associated equilibrium flow, which we call the Condensed DAG equilibrium, exists, is unique, and can be characterized as a strictly convex optimization problem. Moreover, we propose a discrete-time dynamical system that captures a natural adaptation rule employed by self-interested travelers to learn about the emergent congestion on the network. We show that the arc flows generated by this adaptation rule converges to a neighborhood of Condensed DAG equilibrium. To our knowledge, our work is the first to study learning and adaptation in an arc-based TAM. Finally, we present numerical results that corroborate our theoretical results.

==> A0_Brief_Depth_Height.tex <==

\subsection{Definitions related to DAG}
Consider a directed acyclic graph \(\tilde{G}= (\tilde{I},\tilde{A})\), where \(\tilde{I}\) is the set of nodes and \(\tilde{A}\) is the set of arcs. Let \(o,d\in \tilde{I}\) be two distinct nodes that are assigned to be origin and destination respectively. Let \(\tilde{\routes}\) be the set of (simple) routes connecting the node \(o\) with \(d\).  We define the following notions which are crucial for the exposition of this paper:
\begin{itemize}
\item[\textsf{(D1)}] \textbf{Location of an arc on a route:} Given an arc \(a\in \tilde{A}\) and route $r \in \tilde{\routes}$ such that $a \in r$, let $\depth_{a,r}$ denote the location of arc $a$ in route $r$, i.e., $a$ is the $\depth_{a,r}$-th arc on route $r$.
\item[\textsf{(D2)}] \textbf{Depth of an arc:} Given an arc \(a\in \tilde{A}\), we denote the depth of arc \(a\) by \(\depth_{a}\) which satisfies that
\begin{align} \label{Eqn: Def, ell a}
    \depth_a &:= \max_{r \in \tilde{\routes}: a \in r} \depth_{a,r}, 
    % \\ \label{Eqn: Def, ell(G)}
    % \depth(\graphMod) &:= \max_{a \in \arcsMod} \depth_a.
\end{align}
\item[\textsf{(D3)}] \textbf{Maximum depth of the Graph:} The maximum depth of the graph is denoted as \(\ell(G) := \max_{a\in \tilde{A}} \ell_a\).
\item[\textsf{(D4)}] \textbf{Depth of a node:} Given a node \(i\in \tilde{I}\), we define depth of a node to be \(\depthNode_i = \max_{a\in A_{i}^+}\ell_a\).
\item[\textsf{(D5)}] \textbf{Height of an arc on a route:} Given an arc \(a\in\tilde{A}\) and route \(r\in \tilde{R}\) such that \(a\in r\), let \(\height_{a,r}\) denote the height of arc \(a\) on paht \(r\). It is defined to be \(\height_{a,r} = |r|-\depth_{a,r}\).  
\item[\textsf{(D6)}] \textbf{Height of an arc:} Given an arc \(a\in \tilde{A}\), we denote the height of arc \(a\) by \(\height_a\) such that 
\begin{align} \label{Eqn: Def, m a}
    \height_a &:= \max_{r \in \tilde{\routes}: a \in r} \height_{a,r}, 
\end{align}  
\item[\textsf{(D7)}] \textbf{Maximum height of the graph:} The maximum height of the graph is defined to be \(\height(G) := \max_{a\in \tilde{A}} \height_a\)
\item[\textsf{(D8)}] \textbf{Height of a node:} Given a node \(i\in \tilde{I},\) we define the height of the node \(i\) to be \(\heightNode_i := \max_{a\in \tilde{A}_i^{+}} \height_a\)
\end{itemize}

\subsection{Table of Notaions}
\todo[inline]{If there remains any space at the end we should include a table of notations.}

~\\
\frank{I am not sure why this is necessary, and even if it is, why it should be placed here. The notation is already described in Section 2. Moreover, it will be inconvenient for a reader to flip back and forth between the table on this page, and the exposition in the main paper. If we really want a table for notation, we should put it in Section 2, where we first introduce the notation.}
~\\

\chinmay{Yeah, I agree this may not be best place for it, but I think Section 3 will  be better place than Section 2 because we define some more notations in Section 3 like \(z,\varphi\). But at this point I am not very concerned about this as we can only include it if there is space. So may we can discuss about this again on Friday.}

~\\
\frank{Also, do you want part of the appendix in the main paper and part of it in the extended ArXiv version?}

\chinmay{Yeah, I did not have any ideas for good placement for the above definitions in main text. So I thought we can have appendix with main paper and extended appendix wiht the full paper. I think it would better utilize the space we have on page 8. But we can discuss if you have other suggestions for placement of this definition}

==> A4_Sec_5.tex <==

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/phi_dynamics.eps}
    \caption{Latency-to-go $\varphi$ vs. time index $n$ for the Condensed DAG in Figure \ref{fig:Front_Figure___Equivalent_DAG}.}
    \label{fig:phi_dynamics}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/cost.eps}
    \caption{Cost functions for the original traffic network in Figure \ref{fig:Front_Figure___Equivalent_DAG}.}
    \label{fig:cost}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/final_no_toll.eps}
    \caption{No Toll: Steady state MTE flows for the original traffic network in Figure \ref{fig:Front_Figure___Equivalent_DAG}.}
    \label{fig:final_no_toll}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Figures/final_with_toll.eps}
    \caption{With Toll: Steady state MTE flows for the original traffic network in Figure \ref{fig:Front_Figure___Equivalent_DAG}.}
    \label{fig:final_with_toll}
\end{figure}


==> temp.tex <==
% temp.tex


